Disk and Envelope Structure in Class 0 Protostars: I. The Resolved Massive Disk in Serpens FIRS 1

We present the first results of a program to characterize the disk and envelope structure of typical Class 0 protostars in nearby low-mass star forming regions. We use Spitzer IRS mid-infrared spectra, high resolution CARMA 230 GHz continuum imaging, and 2-D radiative transfer models to constrain the envelope structure, as well as the size and mass of the circum-protostellar disk in Serpens FIRS 1. The primary envelope parameters (centrifugal radius, outer radius, outflow opening angle, and inclination) are well constrained by the spectral energy distribution (SED), including Spitzer IRAC and MIPS photometry, IRS spectra, and 1.1 mm Bolocam photometry. These together with the excellent uv-coverage (4.5-500 klam) of multiple antenna configurations with CARMA allow for a robust separation of the envelope and a resolved disk. The SED of Serpens FIRS 1 is best fit by an envelope with the density profile of a rotating, collapsing spheroid with an inner (centrifugal) radius of approximately 600 AU, and the millimeter data by a large resolved disk with Mdisk~1.0 Msun and Rdisk~300 AU. These results suggest that large, massive disks can be present early in the main accretion phase. Results for the larger, unbiased sample of Class~0 sources in the Perseus, Serpens, and Ophiuchus molecular clouds are needed to determine if relatively massive disks are typical in the Class 0 stage.

==> tab1.tex <==
\ProvidesFile{tab1.tex}
\begin{deluxetable}{ccccl}
\tablecolumns{5}
\tablewidth{0pc}
\tablecaption{\label{irstab}\textit{Spitzer} IRS and broadband \textit{Spitzer}, SHARC II, and Bolocam fluxes used in the SED fits}
\tablehead{
\colhead{Wavelength}  & \colhead{Flux} & \colhead{Uncertainty}  & \colhead{Aperture} & \colhead{Instrument} \\
\colhead{($\micron$)}  & \colhead{(Jy)} & \colhead{(Jy)} & \colhead{(arcsec)} & \colhead{} 
}
\startdata
       3.6  & 0.00085  &  0.00016    &  2.2  &  IRAC  \\
       4.5  &  0.0026  &  0.0005     &  2.2  &  IRAC  \\
       5.8  &  0.0023  &  0.0005     &  2.2  &  IRAC  \\
       7.8  &  0.004  &   0.002    &  3.7  &  IRS (SL1) \\
       8.5  &  0.0018  &   0.0010    &  3.7  &  IRS (SL1) \\
       9.1  &  0.0011  &   0.0006    &  3.7  &  IRS (SL1) \\
       9.7  &  0.0002  &   0.0003    &  3.7  &  IRS (SL1) \\
       10.3  &  0.0016 &   0.0008    &  3.7  &  IRS (SL1) \\
       10.9  &  0.0017 &   0.0009    &  3.7  &  IRS (SL1) \\
       11.5  &  0.0024 &   0.0012    &  3.7  &  IRS (SL1) \\
       12.1  &  0.0034 &    0.0017   &  3.7  &  IRS (SL1) \\
       12.7  &  0.005  &    0.003    &  3.7  &  IRS (SL1) \\
       13.3  &  0.005 &    0.002   &  3.7  &  IRS (SL1) \\
       13.9  &  0.006  &    0.003    &  3.7  &  IRS (SL1) \\
       14.5  &  0.007 &    0.003     &  3.7  &  IRS (SL1) \\
       15.0  &  0.0019 &   0.0011    &  3.7  &  IRS (SL1) \\
       15.4  &  0.009 &    0.006     &  10.5  &  IRS (SH) \\
       16.3  &   0.021 &    0.008    &  10.5  &  IRS (SH) \\
       18.1  &   0.033 &    0.010    &  10.5  &  IRS (SH) \\
       19.8  &    0.121 &    0.017   &  11.1  &  IRS (LH) \\
       20.7  &    0.21 &     0.04    &  11.1  &  IRS (LH) \\
       21.7  &    0.36 &    0.04     &  11.1  &  IRS (LH) \\
       22.7  &    0.59 &    0.07   &  11.1  &  IRS (LH) \\
       23.8  &     1.04 &     0.11   &  11.1  &  IRS (LH) \\
       25.1  &     2.0 &     0.2   &  11.1  &  IRS (LH) \\
       26.5  &     3.1 &     0.3   &  11.1  &  IRS (LH) \\
       28.0  &     4.6 &     0.5   &  11.1  &  IRS (LH) \\
       29.7  &     6.8 &     0.7   &  11.1  &  IRS (LH) \\
       31.6  &     9.1 &     1.0   &  11.1  &  IRS (LH) \\
       33.9  &     11.8 &      1.3 &  11.1  &  IRS (LH) \\
       36.0  &     13.4 &      1.5 &  11.1  &  IRS (LH) \\
       70    &     77 &    41    &  17  &  MIPS  \\
       350   &     195 &    79   &  40  &  SHARC II  \\
       1100 &     5.9 &   1.2        &  40  &  Bolocam
\enddata
\tablecomments{
Apertures in which fluxes are calculated correspond to the instrument PSF, with the exception of the SHARC~II and Bolocam fluxes.
Calibrated IRS fluxes are averaged in wavelength bins of $\Delta \lambda \sim 0.75~\micron$, $1~ \micron$, and $1.5~\micron$ for SL1, SH, and LH, respectively, as described in Section~\ref{irsobs}.  The IRS flux is the mean within a bin, and the instrumental uncertainty is the error in the mean ($\sigma/\sqrt{N}$).  All uncertainties include a 10\% systematic uncertainty in addition to the instrumental uncertainty.}
\end{deluxetable}
\endinput


==> tab2.tex <==
\ProvidesFile{tab2.tex}
\begin{deluxetable}{ccc}
%\tabletypesize{\scriptsize}
\tablecolumns{3}
\tablewidth{0pc}
\tablecaption{\label{vistab} CARMA 230~GHz visibilities}
\tablehead{
%\colhead{Wavelength}  & \colhead{Flux} & \colhead{$\sigma_M$} \\
\colhead{$uv$-distance}  & \colhead{Flux} & \colhead{Uncertainty} \\
\colhead{(k$\lambda$)}  & \colhead{(Jy)} & \colhead{(Jy)} 
}
\startdata
       4.50  &     2.45   &    0.12   \\
       7.50  &     2.05   &    0.07   \\
       10.5  &     1.96   &    0.07   \\
       13.5  &     1.70   &    0.06   \\
       16.5  &     1.60   &    0.06   \\
       19.5  &     1.38   &    0.05   \\
       22.5  &     1.31   &    0.05   \\
       25.5  &     1.17   &    0.04   \\
       28.5  &     1.10   &    0.04   \\
       31.5  &     1.07   &    0.04   \\
       34.5  &    0.97   &    0.04   \\
       37.5  &    0.89   &    0.04   \\
       40.5  &    0.86   &    0.04   \\
       43.5  &    0.83   &    0.04   \\
       46.5  &    0.75   &    0.03   \\
       49.5  &    0.73   &    0.04   \\
       52.5  &    0.74   &    0.04   \\
       55.5  &    0.68   &    0.03   \\
       58.5  &    0.77   &    0.04   \\
       61.5  &    0.72   &    0.04   \\
       64.5  &    0.67   &    0.04   \\
       67.5  &    0.61   &    0.04   \\
       70.5  &    0.62   &    0.05   \\
       73.5  &    0.54   &    0.04   \\
       76.5  &    0.52   &    0.04   \\
       79.5  &    0.57   &    0.05   \\
       82.5  &    0.70   &    0.05   \\
       85.5  &    0.71   &    0.06   \\
       88.5  &    0.59   &    0.07   \\
       91.5  &    0.54   &    0.05   \\
       94.5  &    0.67   &    0.05   \\
       97.5  &    0.47   &    0.05   \\
       100.5 &    0.36   &    0.06  \\
   &  \nodata & 
\enddata
\tablecomments{Visibilities and uncertainties used in the model fits. The amplitude bias, or expected value for zero signal, has been subtracted from the data.  [The full table will appear in the online version.] }
\end{deluxetable}
\endinput
%\vspace{0.3in}

